ImageInThat: Manipulating Images to Convey User Instructions to Robots

Foundation models are rapidly improving the capability of robots in performing everyday tasks autonomously such as meal preparation, yet robots will still need to be instructed by humans due to model performance, the difficulty of capturing user preferences, and the need for user agency. Robots can be instructed using various methods-natural language conveys immediate instructions but can be abstract or ambiguous, whereas end-user programming supports longer horizon tasks but interfaces face difficulties in capturing user intent. In this work, we propose using direct manipulation of images as an alternative paradigm to instruct robots, and introduce a specific instantiation called ImageInThat which allows users to perform direct manipulation on images in a timeline-style interface to generate robot instructions. Through a user study, we demonstrate the efficacy of ImageInThat to instruct robots in kitchen manipulation tasks, comparing it to a text-based natural language instruction method. The results show that participants were faster with ImageInThat and preferred to use it over the text-based method. Supplementary material including code can be found at: https://image-in-that.github.io/.

==> camera_ready/sections/0b-teaserfigure.tex <==
\begin{teaserfigure}
  \centering
  % \vspace{-3mm}
  % \includegraphics[width=\textwidth]{figures/teaser/teaser.pdf}
  \includegraphics[width=0.7\linewidth]{figures/Teaser.pdf}
  \missingfigure{Teaser figure}
  % \vspace{-7mm}
  \caption{We present \mk{\projname}, a system for \dots
    \normalfont{  
      \textbf{\textcircled{a}} Caption\dots
    }
  }
  \label{fig:teaser}
\end{teaserfigure}



==> camera_ready/sections/0d-ccs.tex <==
\begin{CCSXML}
    <ccs2012>
        <concept>
            <concept_id>10003120.10003121.10003124.10010392</concept_id>
            <concept_desc>Human-centered computing~Mixed / augmented reality</concept_desc>
            <concept_significance>500</concept_significance>
        </concept>
        <concept>
            <concept_id>10003120.10003121.10003124.10011751</concept_id>
            <concept_desc>Human-centered computing~Collaborative interaction</concept_desc>
            <concept_significance>500</concept_significance>
        </concept>
        <concept>
            <concept_id>10010147.10010371.10010352.10010378</concept_id>
            <concept_desc>Computing methodologies~Procedural animation</concept_desc>
            <concept_significance>500</concept_significance>
            </concept>
      </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Mixed / augmented reality}
\ccsdesc[500]{Human-centered computing~Collaborative interaction}
\ccsdesc[500]{Computing methodologies~Procedural animation}

\keywords{Mixed reality; situated computing; spatial computing;}

==> camera_ready/sections/0f-acm-license.tex <==
\copyrightyear{2023} 
\acmYear{2023} 
\setcopyright{acmlicensed}
%\acmConference[UIST '23]{The 36th Annual ACM Symposium on User Interface Software and Technology}{October 29-November 1, 2023}{San Francisco, CA, USA}
%\acmBooktitle{The 36th Annual ACM Symposium on User Interface Software and Technology (UIST '23), October 29-November 1, 2023, San Francisco, CA, USA}
\acmPrice{15.00}
\acmDOI{10.1145/3586183.3606825}
\acmISBN{979-8-4007-0132-0/23/10}

==> paper-packages.tex <==
% *** Nicer tables ***
% \usepackage{booktabs}
% \newcommand{\tabitem}{~~\llap{\textbullet}~~}
% \usepackage{multirow}
% \usepackage{makecell}
% \renewcommand\theadalign{bc}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[4pt]}
% \renewcommand\cellgape{\Gape[4pt]}
% \usepackage{tabularx}
% \usepackage{array}

% *** Approved packages ***
\usepackage{array}
\usepackage{amsmath}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{float}
% \usepackage{wrapfig}
\usepackage{xspace}
\usepackage{enumitem}
\usepackage[italic]{mathastext}
\setlistdepth{9}

% *** Other packages ***
\usepackage{lipsum}
\usepackage{todonotes}
% \usepackage{tikz}
% \usepackage{adjustbox}
% \usepackage{pdfpages}

\DeclareEmphSequence{\bfseries}


==> paper-settings.tex <==
% SIGRAPH
%%\citestyle{acmauthoryear}

\setlength{\intextsep}{0pt}%
\hyphenation{geo-metri-cally}

%% change title font size
% \makeatletter
% \renewcommand\Huge{\@setfontsize\Huge{12.5pt}{20}}
% \makeatother

% \setlength{\textfloatsep}{5pt}
% \setlength{\floatsep}{5pt plus 1.0pt minus 2.0pt}
% \setlength{\intextsep}{5pt plus 1.0pt minus 2.0pt}

==> sections/0a-authors.tex <==

% \author{Karthik Mahadevan} 
%     \affiliation{%
%     \institution{Department of Computer Science \\ University of Toronto}
%             \streetaddress{}
%             \city{Toronto}
%             % \state{}
%             \country{Canada}
%     }

% \author{Reinhard Sch\"utte}
%     \affiliation{%
%         \institution{Institute for Computer Science \\ University of Duisburg-Essen}
%         \streetaddress{}
%         \city{Essen}
%         % \state{}
%         \country{Germany}
%         \postcode{45141}
%     }

\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}

\renewcommand{\shortauthors}{Anon et al.}

==> sections/0b-teaserfigure.tex <==
\begin{teaserfigure}
  \centering
  % \vspace{-3mm}
  % \includegraphics[width=\textwidth]{figures/teaser/teaser.pdf}
  \includegraphics[width=0.7\linewidth]{figures/Teaser.pdf}
  \missingfigure{Teaser figure}
  % \vspace{-7mm}
  \caption{We present \mk{\projname}, a system for \dots
    \normalfont{  
      \textbf{\textcircled{a}} Caption\dots
    }
  }
  \label{fig:teaser}
\end{teaserfigure}



==> sections/0c-abstract.tex <==
\begin{abstract}
    Foundation models are rapidly improving the capability of robots in performing everyday tasks autonomously such as meal preparation, yet robots will still need to be instructed by humans due to model performance, the difficulty of capturing user preferences, and the need for user agency. Robots can be instructed using various methods---natural language conveys immediate instructions but can be abstract or ambiguous, whereas end-user programming supports longer-horizon tasks but interfaces face difficulties in capturing user intent. In this work, we propose using direct manipulation of images as an alternative paradigm to instruct robots, and introduce a specific instantiation called \projname which allows users to perform direct manipulation on images in a timeline-style interface to generate robot instructions. Through a user study, we demonstrate the efficacy of \projname to instruct robots in kitchen manipulation tasks, comparing it to a text-based natural language instruction method. The results show that participants were faster with \projname and preferred to use it over the text-based method.
\end{abstract}

% We demonstrate that it is possible to translate image-based instructions into executable robot code and discuss the potential of blending the strengths of language and images to create multimodal robot instructions. 

% We demonstrate how \projname can be used to execute robot actions and discuss how language and image can be blended to create multimodal robot instructions.

==> sections/0d-ccs.tex <==
\begin{CCSXML}
    <ccs2012>
        <concept>
            <concept_id>10003120.10003121.10003124.10010392</concept_id>
            <concept_desc>Human-centered computing~Mixed / augmented reality</concept_desc>
            <concept_significance>500</concept_significance>
        </concept>
        <concept>
            <concept_id>10003120.10003121.10003124.10011751</concept_id>
            <concept_desc>Human-centered computing~Collaborative interaction</concept_desc>
            <concept_significance>500</concept_significance>
        </concept>
        <concept>
            <concept_id>10010147.10010371.10010352.10010378</concept_id>
            <concept_desc>Computing methodologies~Procedural animation</concept_desc>
            <concept_significance>500</concept_significance>
            </concept>
      </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Mixed / augmented reality}
\ccsdesc[500]{Human-centered computing~Collaborative interaction}
\ccsdesc[500]{Computing methodologies~Procedural animation}

\keywords{Mixed reality; situated computing; spatial computing;}

==> sections/0e-acks.tex <==
\begin{acks}
    We thank \mk{\dots}.
\end{acks}

==> sections/0f-acm-license.tex <==
\copyrightyear{2023} 
\acmYear{2023} 
\setcopyright{acmlicensed}
%\acmConference[UIST '23]{The 36th Annual ACM Symposium on User Interface Software and Technology}{October 29-November 1, 2023}{San Francisco, CA, USA}
%\acmBooktitle{The 36th Annual ACM Symposium on User Interface Software and Technology (UIST '23), October 29-November 1, 2023, San Francisco, CA, USA}
\acmPrice{15.00}
\acmDOI{10.1145/3586183.3606825}
\acmISBN{979-8-4007-0132-0/23/10}

==> sections/1-introduction.tex <==
\section{Introduction}

% \bla{I think this paragraph justifies the need for user intervention versus a fully autonomous ``interaction'', but I think it should instead spend one sentence justifying that, and more sentences justifying why more methods for creating and interpreting instructions for robots are needed. I.e. issues with representing instructions with language, or end user programming. I also think the reasons for needing user intervention are multifaceted, and more than just generic models don't adapt to user preferences. I think there's other issues such as models not actually performing well enough, and I think there's likely a user desire for more control over the model https://dl.acm.org/doi/abs/10.1145/3290605.3300750}. 

Advances in foundation models are rapidly improving the capabilities of autonomous robots, bringing us closer to robots entering our homes where they can complete everyday tasks. However, the need for human \textit{instructions} will persist---whether due to limitations in robot policies, models trained on internet-scale data that may not capture the specifics of users' environments or preferences, or simply the desire for users to maintain control over their robots' actions. For instance, a robot asked to wash dishes might follow a standard cleaning routine---\textit{e.g.}, by placing everything in the dishwasher and then putting them away in the cupboard---but may not respect a user's preferences---\textit{e.g.}, needing to wash delicate glasses ``by hand'' or organizing cleaned dishes in a specific way---thus necessitating human intervention.

Existing methods for instructing robots range from those that focus on \textit{commanding} the robot for the purpose of immediate execution (\textit{e.g.}, uttering a language instruction to wash glasses by hand~\cite{lynch2023interactive}) to methods that \textit{program} the robot such as learning from demonstration~\cite{argall2009survey} or end-user robot programming~\cite{ajaykumar2021survey}. However, prior methods, whether they are used for commanding or programming, have notable drawbacks. Using language to command a robot can be quick and generate an immediate execution from the robot, although language can be abstract and difficult to ground in the robot's environment. For instance, the command \textit{``put away the dishes in the cabinets after cleaning them''} is ambiguous if there are dishes of different types, each needing to be placed in different areas of the same cabinet or in entirely different cabinets. End-user programming promotes the creation of reusable programs for repeated execution, yet it remains challenging to capture user intents~\cite{ajaykumar2021survey}.

% However, these
% abstractions still require an understanding and explicit speci￿cation
% of the programming logic which presents a signi￿cant barrier.

%\mk{Computers \dots}
%The advancement of large foundation models that process combination of language and vision has made robots more intelligent and capable of performing complex tasks.
% \bla{If our goal is to position images in the landscape of techniques for instructing robots, I think we should stray away from comparing to language so much and instead make a general claim that the underlying problem we are solving are *many* drawbacks across different methods of instructing. For instance, interpreting end user programs is very difficult, language is difficult because of ambiguity, teleop requires an immense amount of concentration and has primarily been explored for real-time tasks not future tasks. The time spent manipulating for teleop is 1-1, so why wouldn't you do household tasks yourself.}

% As it is expected that most users of future robots will not be experts, natural language has been touted as a modality that people can use to instruct robots~\cite{tellex2020robots}. From a technical standpoint, state-of-the-art robot policies often utilize language-conditioning to generate robot actions. Despite the ubiquity of language and its easy-to-use interface, language is not always ideal. Natural language can be abstract and difficult to ground in the physical context. For instance, \textit{``Put the cereal in the cabinet'' }is unclear if there are many boxes of cereal and several cabinets to put them away inside of. Hence, the user needs to be more precise to achieve the desired result: \textit{``Put the blue cereal box into the top left corner of the middle cabinet next to the other cereal''}, or alternatively, provide corrections to a simpler instruction by uttering language~\cite{zha2023distilling}. Beyond the immediate problem of specifying instructions, the user faces the additional challenge of predicting how the robot's planned actions will affect the environment, particularly for long-horizon tasks.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/Group 44.pdf}
    \caption{We introduce the direct manipulation of images as a paradigm for providing instructions to a robot. Depicted in the bottom left are a series of instructions that a user is giving the robot by manipulating the fruits. The top shows one trajectory of direct manipulation}
    \label{fig:enter-label}
\end{figure}

In this paper, we propose directly manipulating images on a visual interface as a means of instructing a robot. By \textit{images}, we mean a visual observation of the robot's environment captured by a camera attached to the robot or the environment. Similar to how cleaning robots today present a visual map of their surroundings, we envision future robots offering access to image observations of the robot's environment. Compared to prior methods for instructing robots, images are easy to interpret, even for longer horizon tasks, since they are already grounded in the robot's environment. Moreover, direct manipulation~\cite{shneiderman1983direct} inherently reduces ambiguity, as actions such as manipulating an object within the image eliminate the need for descriptive instructions~\cite{masson2024directgpt}. We introduce a specific instantiation of this paradigm, \projname, which combines many state-of-the-art foundation models, and enables users to manipulate images of the robot's environment to create instructions. \projname integrates several techniques:
\begin{itemize}
    \item \textit{Direct manipulation} of objects and fixtures to create instructions;
    \item A \textit{timeline interface} for ordering instructions and assessing whether the shown changes achieve them;
    \item \textit{Highlighting changes} between instructions using visualization methods to help users interpret changes; 
    \item \textit{Language-based image editing} to leverage the strengths of language to visualize instructions;
    \item \textit{Automatic captioning} of user manipulations with text to enhance confidence about the robot's understanding of instructions;
    \item \textit{Predicting and proposing future instructions} based on contextual interpretation of user actions.
\end{itemize}

In a user study with ten participants, we compared \projname to a language-based method for four instruction-following tasks in simulated kitchen environments. We found that participants were able to generate instructions in these tasks faster (64.8\% less time) when using \projname, and participants were more confident that their instructions could be understood by a robot when they directly manipulated images to provide instructions. We further demonstrate that image-based instructions created using \projname can be translated and executed on a physical robot arm through a case study. This work advances the state-of-the-art by making the following contributions:
\begin{itemize}
    \item An alternative paradigm of instructing robots enabled by the direct manipulation of images on a visual interface;
    \item An instantiation of this paradigm, \projname, realized through a novel prototype;
    \item Results of a user evaluation comparing \projname to an instance of a language-based method;
    \item Early demonstrations that user-generated images can be translated into robot actions.
\end{itemize}


==> sections/2-background.tex <==
\section{Background}
Prior robotics literature has proposed several paradigms using which humans can instruct robots. Broadly, these can be categorized as \textit{commands}--instructions that are provided and executed in the moment, and \textit{programs}--structured instructions that can be repeated in an automated fashion. Regardless of whether a robot is instructed through commands or a program, instructions require four major components: (1) capturing user intent, (2) translating that intent into a command or program, (3) presenting the command or program to the user for confirmation or feedback, and (4) executing the instruction.

%they all inherently have a representation and can incorporate three major aspects to support the user: \textit{creation}, \textit{interpretation}, and \textit{execution}.

%We view instructions from the user side as requiring three components: the ability to \textit{represent} the instruction in a way that the user can interpret it, 
%create, represent, and execute instructions.

\noindent \emph{Continuous commands}. Commands can be issued in real-time or near real-time (referred to as control in the robotics literature) and involve continuous input from the user through \textit{teleoperation}, for which several methods exist. Since continuous commands are typically executed in real-time, there is often no explicit notion of presenting user intent for confirmation or feedback (3), For instance, when using a physical device for teleoperation~\cite{gopinath2016human, temma2019third}, manipulating the device captures user intent to provide specific changes (deltas) to the robot's end effector pose or joint configuration, whereas execution occurs immediately through low-level controllers~\cite{darvish2023teleoperation,rea2022still}. The user gets feedback implicitly but in real time while the robot executes the command---by either observing the robot after executing a command physically~\cite{rakita2020effects} or visually during remote teleoperation~\cite{wei2021multi,naceri2019towards,rakita2018autonomous}. In contrast, graphical user interfaces often provide the user feedback prior to execution, such as by visualizing valid commands~\cite{kent2017comparison, li2020starhopper,rosen2020communicating}, virtual surrogates that can be manipulated instead of the real robot~\cite{walker2019robot,quintero2018robot, mahadevan2022mimic}, or visualizing and manipulating a 3D rendering of the robot's environment in 3D~\cite{li2022scene,aoyama2024asynchronously}. 

\noindent \emph{Discrete commands.} Other methods of issuing commands provide a layer of abstraction to reduce the user burden of having to provide continuous input. For instance, users can create instructions through natural language which are executed immediately~\cite{matuszek2013learning, lynch2023interactive, tellex2020robots}. Although this abstraction provides the opportunity for user feedback, it is often not utilized and the user interface is simply the language used (\textit{e.g.,} natural language). Some recent work provides the opportunity for user intervention via language as an interface, such as where the robot engages in a dialogue to clarify instruction ambiguities ~\cite{huang2022inner}, requests user help~\cite{ren2023robots}. or lets the user provide iterative language corrections~\cite{zha2023distilling, liang2024learning}. From an execution standpoint, discrete commands such as those that are language-based can be executed by pretrained general-purpose large language models (LLMs) that translate them into policy code~\cite{liang2023code, singh2023progprompt, liu2024ok, mahadevan2024generative} or in an end-to-end fashion using trained special-purpose robot foundation models that map language to robot actions~\cite{lynch2023interactive, brohan2022rt, team2024octo, kim2024openvla}.

\noindent \emph{Programs.} Prior work has proposed methods to create instructions for longer-horizon tasks in a repeatable manner, and employ a variety of instruction representations. Graphical programming representations, such as blocks~\cite{huang2017code3, huang2016design, weintrop2018evaluating} and nodes~\cite{alexandrova2015roboflow,porfirio2018authoring}, are often used in end-user robot programming (EURP) systems. Other approaches utilize augmented reality~\cite{ikeda2024programar, suzuki2022augmented, quintero2018robot, gong2019projection, cao2019ghostar}, sketching~\cite{sakamoto2009sketch, porfirio2023sketching}, and tangibles~\cite{sefidgar2017situated, gao2019pati, porfirio2021figaro}. Recently, LLMs have been employed to enable the use of freeform natural language to create text-based programs using chat interfaces~\cite{karli2024alchemist, ge2024cocobo}. The creation step of a program involves defining the step-by-step procedure of the robot's behavior, for instance by dragging-and-dropping individual blocks in a visual editor~\cite{huang2017code3}. 

Since EURP is typically done offline, most systems enable the user to provide confirmation to the system and gather feedback using a given representation. For instance, blocks in a program can be viewed in a visual editor whereas other methods contextualize the program such as with augmented visualizations on a tabletop~\cite{gao2019pati, sefidgar2018robotist} or mapping the robot's environment within the editor~\cite{huang2020vipo}. This helps track the robot's future states and identify possible errors. Beyond viewing and confirmation steps, most EURP systems support editing instructions natively. Programs are often executed using classical methods such as motion planning~\cite{gao2019pati} or program synthesis~\cite{porfirio2019bodystorming}. However, LLMs have also recently been employed to generate code from a program~\cite{karli2024alchemist}. 

Our work does not distinctively fit into either paradigm, but borrows from and has applicability to both. We also utilize an instruction representation, namely, images, which has been less explored for instructing robots, particularly for the end user. Using images as a representation offers several benefits. Instructions can be created quickly through direct manipulation, is concrete by nature (since manipulation occurs on a specific object of interest), and reduces ambiguities that are inherent to other methods (\textit{e.g.}, language). This approach can be used to \textit{command} a robot in near real time (akin to language). Further, because images are concrete, they can help the user in tracking the robot's state over time. Hence, it can support the creation of procedures for longer-horizon tasks as with \textit{programming}. Lastly, using images as a representation supports flexible execution, such as by translating images to robot policy code~\cite{liang2023code} (which we demonstrate in this work), and potentially translating images into language captions for executing trough language-conditioned policies~\cite{kim2024openvla}, or immediately used via image-conditioned policies~\cite{team2024octo}.

% We present a small model and mini taxonomy in which these paradigms fit into, and argue that beyond these paradigms there is a generalisable concept regarding robot instruction. Whether the user is trying to program the robot, live control it, or use instruction following, the instruction the user is conveying MUST be created and represented in some manner. Teleoperation uses a live video, end user programming ranges from using blockbased programming, instruction following creates the representation with voice and interprets it with sound or written text. In this paper we use a static 2D image of the environment both to manipulate and create instructions for the robot. % In the remaining background and related work we discuss the projects which are most similar to our work, and a brief survey of different methods of the modalities used to create, represent, and execute instructions.(show less)

% \noindent \emph{End-user robot programming.} Prior EURP work can be largely categorized into natural language-based and visual-based methods. Many systems employ speech for programming~\cite{cakmak2014teaching, gorostiza2011end}, though challenges remain in recognition and creating complex programs through continuous dialogue. Other approaches use text-based programming with visual scaffolds like blocks~\cite{huang2017code3, huang2016design, weintrop2018evaluating} or nodes~\cite{alexandrova2015roboflow,porfirio2018authoring}. Recently, large language models (LLMs) have been employed for text-based interactions, often via chat interfaces~\cite{karli2024alchemist, ge2024cocobo}. However, language input demands precision, especially for spatial tasks in robotics~\cite{masson2024directgpt, sundaresan2024rt}. Other systems span a range of visual modalities, such as augmented reality~\cite{ikeda2024programar, suzuki2022augmented, quintero2018robot, gong2019projection, cao2019ghostar}, spatial interfaces~\cite{huang2020vipo, cao2019v, mahadevan2022mimic}, sketch-based systems~\cite{sakamoto2009sketch, porfirio2023sketching}, physical demonstrations~\cite{akgun2012trajectories}, and tangible interaction~\cite{sefidgar2017situated, gao2019pati}. Despite the richness of prior EURP systems, they often require adherence to specific system rules. For instance, AR-based trigger-action programming~\cite{ikeda2024programar} necessitates precise trigger and action specifications within the user's AR environment. Moreover, many prior systems use intermediate representations (e.g., flow diagrams or blocks) to convey user intent. In contrast, \projname enables users to directly manipulate images to represent a desired world state without an intermediate representation.

%  There are also interfaces that provide some assistance such as for switching control modes autonomously~\cite{herlant2016assistive} or through user instructions~\cite{cui2023no}.

% Both teleoperation and instruction following require a human-in-the loop which reduces their ability to support users in offloading their tasks to the robot. 

% \noindent \emph{Live robot control.} Modern robotic systems often include interfaces for the real-time teleoperation of the robots' joint and end-effector positions.
% These interfaces are often based on graphical user interfaces (GUIs) or joysticks, offering immediate feedback for the controllers to adjust their input~\cite{darvish2023teleoperation,rea2022still}.
% While effective, GUI- and joystick-based control mechanisms are cognitively and physically taxing for human operators, as they demands mental rotation and managing multiple separate degrees of freedom (DoFs) simultaneously.
% To alleviate this burden, one thread of recent teleoperation research aims to directly map human motion to robot motion, often from the motion of human hands to robot end-effectors~\cite{rakita2017motion,rakita2019shared,fu2024mobile}.
% Other work opts for a shared-control approach, where some trajectory prior informs a robot to generate high DoF trajectories from low DoF input.
% Such prior is often derived from inferred operator goals~\cite{huang2016anticipatory,jain2019probabilistic,losey2022learning}.
% Despite the assistance available, live control methods still require operators' continuous mental and physical engagement to manage robots' low-level motion.
% Therefore, \projname, along with other recent research, seeks to enable robots to interpret and execute human operators' high level intents.


% creation, interpretation, and execution. 


% Added \bla{there is a commented out attempt at framing this as background and related work below here.} \bla{The goal of the rewrite is to argue that all forms of robot instruction (end user programming, instruction following, live control, etc.) rely on some form of instruction representation. We do not want our work to be seen as end user programming, and it's definitely not live control. But we don't want to introduce our own paradigm. That's a big leap. Instead, we introduce the abstract notion of \textit{Instruction Representation}, which covers many of these areas, and argue that there are three important aspects namely: creation, interpretation, and execution. And then we can argue that representing instructions as images has key benefits, and those benefits might apply to other paradigms as well.}

% The HRI literature includes several paradigms in which a human might instruct a robot. For example, humans might use *teleoperation* where they are interacting in real time and directly controlling the robots movement, or *live control* which is also done synchronously in real-time, however the method used to control the robot is typically abstracted, perhaps using instruction following and voice to control the robot and give language based commands. The feedback loop in these cases is so tightly integrated that the instructions are usually not represented to the user in any other way than by using an image of the environment. These approaches are rooted in the real-time nature. % However, our application domain attempts to address problems in the household where a user might want to offload tasks. If these were done in real time with a human in the loop then it is difficult to imagine the user would be saving time. Some paradigms have attempted instruct robots in a non-real time manner. For example, end-user robotics programming tries to create reusable programs that the robot can execute. % Our paper does not fit directly into any of these paradigms, and instead represents a combination of many of them. We take from the end user programming literature the idea of constructing many consecutive steps, but from instruction following and live control we take the representation of instructions. It is unclear where this new paradigm sits, but it is somewhere at the intersection of end user robotics programming and instruction following. % We present a small model and mini taxonomy in which these paradigms fit into, and argue that beyond these paradigms there is a generalisable concept regarding robot instruction. Whether the user is trying to program the robot, live control it, or use instruction following, the instruction the user is conveying MUST be created and represented in some manner. Teleoperation uses a live video, end user programming ranges from using blockbased programming, instruction following creates the representation with voice and interprets it with sound or written text. In this paper we use a static 2D image of the environment both to manipulate and create instructions for the robot. % In the remaining background and related work we discuss the projects which are most similar to our work, and a brief survey of different methods of the modalities used to create, represent, and execute instructions.(show less)


% If I were you, I would go with the latter option of broad comparison. I see your concern that people might see these as apples and oranges, but there is also the risk that some people will see instruction as being similar to programming and think that you are ignoring this whole other approach/body of work.

% The way I see is that we either give robots commands (to be executed there and then, and only once) or program them (to repeatedly do something in an automated fashion). Commands generally include natural language and teleoperation, programming include learning (in its various forms) and end-user programming. I think that your method has applicability and relevance to all of these methods. It can be used to command a robot or program a robot (either as input into learning or end-user programming).

% Of course, covering a wide body of related work may be a challenge, but you could perhaps limit it to one subsection of RW and touch on all these methods.

==> sections/4-approach.tex <==
\begin{figure*}[htbp]
%% Size
\centerline{\includegraphics[width=0.7\textwidth]{figures/Interface.pdf}}
\caption{\projname's user interface, consisting of an editor (top) and a timeline (bottom). The editor allows users to manipulate objects and fixtures in the environment, while the timeline displays the current state of the environment and the desired changes. The timeline (B) shows all instructions to the robot. Selecting a step populates it in the editor (B). Changes between steps are made visible by contrasting changed objects and fixtures from other items (C). \projname automatically captions all manipulations and allows them to be edited. The user can instruct the robot with text to generate new steps automatically. \projname tries to predict user goals such as by proposing locations where objects can be placed (F) or predicting a future step (G).}
\label{fig:interface}
\end{figure*}

\section{Image Manipulation through ImageInThat}
%% These assumptions are justified, as any robot entering a new environment would undergo an initialization phase to understand its surroundings. However, this knowledge can also be provided by the user or inferred by other models. 
We introduce manipulating images as a new way to instruct robots. Here, we describe the interactions that a user can have with \projname, a prototype instantiation of this concept. To enable these interactions, \projname assumes that there will be a setup phase where the robot builds an internal representation of the user's environment in which it will operate. This representation consists of knowledge about objects and fixtures. \textit{Objects} are items that can be manipulated from one location to another (\textit{e.g.}, bowls that need washing) whereas \textit{fixtures} are items that are immovable. Both objects and fixtures can be in more than one state; for example, a cabinet is a fixture that can be open or closed. Throughout our description of the \projname system, we will use an example of how a user might have their robot take a particular bowl out of a cabinet that they wish to use to hold an apple by utilizing \projname. To support the creation of new instructions, \projname includes an editor.

\noindent \emph{Direct manipulation to interact with objects and fixtures (\autoref{fig:interface}A.} In the \projname interface, the user can perform simple drag-and-drop operations in the editor to manipulate their locations upon selecting them. The user can also change the order in which objects appear by right clicking them. They can toggle the state of fixtures by clicking on them if they take on a discrete number of states. Here we use the example of instructing the robot to take a bowl from a cabinet to show how the user can manipulate objects and fixtures to construct commands. This task can be decomposed this into three \textit{steps}: (1) open the cabinet; (2) choose a bowl, and move it from the cabinet to the counter; and (3) close the cabinet. In \projname, specifying each of these steps is achieved by performing clicking to toggle between the fixture's states (opening and closing the cabinet) and drag-and-drop operations (moving the bowl). This concreteness is in contrast to prior methods for instructing robots that can inherently contain ambiguities.

\noindent \emph{Timeline to interpret the continually changing environment (\autoref{fig:interface}B).} \projname provides a visual timeline to help the user anchor and understand their instructions to the robot in the context of the continually changing environment. This is especially useful for longer-horizon tasks. When the user opens the interface, the initial state of the environment is pre-populated in the timeline. This serves as the starting point for all instructions for the robot, and future steps represent changes from this initial step. Each step in the timeline is displayed from left to right (temporally) as small thumbnail images. When the user selects a step, it becomes populated inside the editor and available to be modified. Each time the user toggles the state of a fixture by clicking it, a new step is inserted after the current step in the timeline. In a similar manner, every time the user performs a drag-and-drop manipulation on a new object, the timeline is populated with a new step. Continuously manipulating the same object allows the user to refine the object's position without creating unnecessary steps. Sometimes, a set of instructions might involve the same object moving in the environment, such as when a dirty bowl needs to be taken from the counter and rinsed under running water before being placed inside a sink. To support creating such instructions, the user can copy a step from the timeline by selecting a button that appears under the step. They can also delete steps using a button under the step in the timeline. The timeline highlights another benefit of images---the ability to visually track how the robot will manipulate the environment to perform instructions rather than having to imagine it.

\noindent \emph{Visually highlighting changes.} Since images are information dense, and the timeline can hold many images at a time, na\"ively placing images in the timeline may not help the user visually track their instructions over time. To assist with this, \projname utilizes two visualizations. First, each time a step is populated in the timeline, \projname's internal representation already maintains a log of \textit{changes} between consecutive steps. When an object is moved between consecutive steps, it is visually highlighted while all other objects and fixtures are made less salient (\autoref{fig:interface}C). In contrast, when a fixture's state changes, the environment is made more visible (where the fixture is located) by keeping it at full opacity and making all objects less visible. This allows users to quickly scan the timeline and gauge what has changed at each step. When a step is selected, hovering over any previous or future step displays the difference through an animation, showing any changes in object positions and fixture states.

\noindent \emph{Blending language and image.} Image manipulation has the benefit of being concrete. For instance, the manipulation of individual objects may cause them to move to a new location. As an example, the user may wish to put an apple into the bowl they took out of the cabinet. However, since direct manipulation only lets the user move the apple on top of the bowl (as there is no way for it to be put ``inside'' without simulating physics), the user may be unsure whether the robot has understood their instruction. \projname automatically annotates each step using a \textit{caption} (\autoref{fig:interface}D). Captions describe the change between the current step and the previous step. A caption for moving the apple might read, ``\texttt{Move the apple from the cabinet into the bowl}.'' By default, an image and its corresponding caption within the same step are linked together. Hence, any changes to the caption will also modify the image. The user can also modify a caption to provide additional context about the intent of their manipulation to the robot by unlinking the caption from the corresponding image within the step. For instance, the user might want to specify that apples should only be inside the bowl after they have been washed. 

There are also many situations where the user has a higher-level goal (\textit{e.g.}, doing the dishes) but either does not know the sequence of steps needed to achieve the goal or does not want to specify them by hand. \projname allows the user to input a language instruction when a step is selected and populated in the editor (\autoref{fig:interface}E). Depending on the specificity of the instruction, one or many steps, each containing an image describing the change, are automatically generated and populated in the timeline. 

\noindent \emph{Predicting user goals.} Guided by the initial setup phase, \projname determines the locations of all objects and fixtures. It uses this knowledge to propose goal locations for a selected object (\autoref{fig:interface}F). For instance, when the user selects the apple, \projname could propose placing it inside the sink (for washing before use) or inside the bowl (for storing). These choices are visualized as lines originating from the selected object. Selecting any part of the line performs the manipulation for the user instead of requiring a drag-and-drop operation. \projname keeps track of all steps that are populated in the timeline. It uses the contextual information embedded in the timeline to predict what the user might want to do next, and proposes these as plausible next steps outside the timeline (\autoref{fig:interface}) that the user can choose between (\textit{e.g.}, two options). Selecting a plausible step adds it to the timeline while allowing the user to reject one or all plausible steps.

%%%% Types of autocomplete
% Proposing next steps based on existing steps - useful
% Using object selection or current step to propose text (when using input bar) - less useful
% Taking an interaction done by the user (e.g., dragging plate to sink) and proposing an action (drag x to y) automatically (ripped from Damien)
% Proposing the step when an item is selected inside the current step (e.g., plate selected -> can go to cabinet, sink, counter??)


%% What interactions are possible; for now drag/drop + click to change states


% Reg drag and drop 

% Articulated objects



% Autocomplete features


%\subsection{GIFs}


==> sections/5-implementation.tex <==
\section{Implementation}
\noindent \emph{High-level system design.} \projname consists of two major components: (1) a \textit{back-end server} that manages machine learning models to generate the image representations for user manipulation and enables features such as automatic captioning, and (2) a \textit{user interface} for viewing and editing the images, enabling users to create robot instructions. The server is realized as a Flask application that enables two-way communication between the models and the interface. The models are hosted as TCP sockets on workstations within the local network and communicate with the Flask server to respond to requests from the interface. The user interface is built using ReactJS. Our implementation for the user study utilizes images from kitchen environments created using Robocasa~\cite{nasiriany2024robocasa} whereas the real-world deployment uses streamed camera images. \projname uses GPT-4o (gpt-4o-2024-05-13) as the large-language-model (LLM) for producing captions, enabling language-based image edits, and predicting user goals, though this can be swapped for other foundation models. Please see the appendices for more details.

\projname creates an initial representation of the robot's environment by extracting information about the objects and fixtures. \projname assumes access to a predefined list of plausible objects and fixtures plus their states (\textit{e.g.}, a drawer being able to open or close).
While the information about object and fixture is predefined in our implementation, it could also be inferred through automated methods that detect object presences, states, and possible articulation (e.g.~\cite{kerr2024robot,alayrac2017joint,qian2022understanding}). 
%The initial state of fixtures also needs to be defined (but could also be inferred using vision language models).

\noindent \emph{Creating the initial representation for user manipulation.} In \projname, fixture states are realized as background images while object masks are overlaid on top of them. Each combination of states is used to generate an image representing the environment in that state. For example, in a kitchen environment with a drawer and a cabinet, one possible state is the drawer being open while the cabinet remains closed. In the user study, the images are generated by API calls to Robocasa to modify the fixtures aided by generated code from the LLM whilst hiding all objects. We argue that this is a reasonable assumption given that many existing robot applications assume the existence of digital twins~\cite{li2024evaluating}. We also experimented with fine-tuning language-conditioned diffusion models~\cite{brooks2023instructpix2pix, black2023zero} to generate images where fixtures change state using a language prompt for environments that do not have a digital twin. For these environments, the parts of the background behind the objects are reconstructed using inpainting techniques~\cite{elharrouss2020image}.

To enable the direct manipulation of objects, \projname must identify and create masks for them. To achieve this, the LLM is prompted to produce a list of visible items in the environment from the list of plausible ones. Then, an open vocabulary object detector (OwLv2~\cite{minderer2024scaling}) finds the corresponding bounding boxes for both objects and fixtures. Object bounding boxes are then processed using Segment Anything~\cite{kirillov2023segment} to generate masks. For detected fixtures, \projname generates interactable regions using the bounding boxes produced by the object detector, enabling mouse clicks within these regions to activate state changes. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/system.pdf}
    \caption{System diagram of \projname showing its major components. The server side handles the preprocessing step and all intelligent features that require interfacing with the LLM (\textit{e.g.}, autocomplete, captioning, and language to step generation. The client is a web user interface built with ReactJS.}
    \label{fig:enter-label}
\end{figure}

\noindent \emph{Initializing the environment.} After generating backgrounds as well as representing objects and fixtures, the server transmits an environment object and the initial state to the user interface. The environment object represents all static aspects of the environment, including all objects plus their bounding boxes, fixtures with their bounding boxes and their possible states, and the backgrounds corresponding to all fixture state combinations. The initial state, on the other hand, describes the initial location of all objects (\textit{i.e.}, \textit{x} and \textit{y} position) and the states of all fixtures. The user interface renders the initial state of the environment as a step in the timeline represented as an SVG image. In this initial state, object order is also determined using the LLM, whereby receptacles (\textit{e.g.}, bowls) are behind other objects (\textit{e.g.}, fruits). Once the environment is populated, the user can interact with the environment by manipulating objects and fixtures. Each time the user interacts with the environment, new environment states are created (or existing states are updated) to keep track of the locations and states of the fixtures, which subsequently adds new visual steps to the timeline. Changes between steps are displayed by applying filters to the difference between their environment states.

% After processing the initial state of all fixtures, the background image, generated masks, and bounding boxes for the fixtures are sent to user interface and rendered as a an SVG image inside a step. When the user clicks the initial step, the underlying representation is rendered inside an image editing application (\mk{CITE website}). The editor enables simple interactions such as the selection, deselection, and manipulating individual objects. When the user performs direct manipulations on one or more objects, the system creates a new step by copying the representation of the previous step while updating data about any objects that moved. To enable interactable fixtures, bounding boxes containing the location of fixtures are utilized to detect mouse clicks within this region, which activates a state change. When changing state, the current state variable is updated and the corresponding background image is retrieved and utilized when creating the step.

\noindent \emph{Blending language and image.} Each time a new step is created through a drag-and-drop manipulation, the LLM is prompted with data about the environment, environment states at each step, and the corresponding images to generate a caption. For fixture state changes, captions are created simply by appending the object type and the state. 


\begin{figure*}[t]
    \centering
    \includegraphics[width=.7\linewidth]{figures/tasks.pdf}
    \caption{Tasks performed by participants in the evaluation (left to right): \textit{organizing pantry}, \textit{sorting fruits}, \textit{cooking stir-fry}, and \textit{washing dishes}. Depicted here is the environment state at the \textit{beginning} of each task.}
    \label{fig:tasks}
\end{figure*}

When the user enters a language instruction while a step is selected, the data about the environment, the corresponding environment state, and the corresponding image are used to prompt the LLM to classify the instruction as either requiring a fixture state change or an object manipulation. Depending on the result, a subsequent call is made to the LLM to either produce an updated list of fixture states, or manipulate the 2D coordinates of the corresponding object(s). Editing a step's caption produces an updated step using the same approach. By default, just a single step is created with the user's instruction. \projname also supports adding more abstract instructions (\textit{e.g.}, wash the dishes) that can be further broken down into smaller instructions, each producing a step.

\noindent \emph{Predicting user goals.} During pre-processing, the LLM is prompted to filter objects in the environment that can be manipulated by the robot, and all the locations they could be placed. This is used to propose goal locations when the user selects an object. Lastly, to propose plausible steps, the user can press a button near the editor to prompt the LLM with the environment plus all environment states corresponding to all steps until the selected step as well as the corresponding images, with the goal of generating any number of plausible actions (a system parameter) based on the robot's existing skills and the sequence of steps in the timeline. Each action is used to generate a plausible step by determining whether it requires a fixture state change or an object manipulation.

%Before the user begins providing instructions to the robot, \projname creates this initial representation to represent all objects and fixtures that are present in the environment, and determines the initial state. We assume access to the initial state of fixtures in the environment, such as the presence and number of cabinets, drawers, and sinks. For instance, a sample initial state could 

%This step can either be performed manually by a user when introducing their robot to their home, or automatically using models. 

% Describe how we make this by enumerating states 

% Sim/Susie/GPT

% How we make masks

% How we make interactable regions


==> sections/6-evaluation.tex <==
\section{Evaluation} 
We evaluated \projname through a user study conducted in a laboratory with ten participants recruited using university and professional networks $M=25.9$ years, $SD=3.38$ years (5 women, 5 men) who rated their familiarity with providing instructions to a robot on a seven-point Likert scale ($M=4.1$, $SD=2.1$). In the study, we compared an instance of \projname with a language-based method. 

\noindent \emph{Conditions.} To allow a comparison of each modality, we omitted all the language features of \projname, including the ability to generate new images using language instructions or modify them using captions. For the language condition, we re-purposed \projname, replacing all image-based interactions with text. Instead of populating images in the timeline, the user populates the timeline with textual descriptions of task steps. In both conditions, participants provided instructions pertaining to one object at a time, reflecting the current capabilities of robots, which typically limited to single-object manipulation. Further, most language-conditioned robot policies (\textit{e.g.}, ~\cite{kim2024openvla}) follow a similar approach, executing single language instructions at a time. While LLMs can interpret more abstract instructions and decompose them, they may make mistakes that require corrections~\cite{zha2023distilling}.

\noindent \emph{Study design and tasks.} The study utilizes a within-subjects design with two conditions--image and text--that are presented in a counterbalanced order to minimize ordering effects. Within each condition, participants completed four tasks where they instructed a robot to complete kitchen manipulation tasks. The tasks ranged in difficulty from easy to hard: \textit{storing pantry}, \textit{sorting fruits}, \textit{cooking stir-fry}, and \textit{washing dishes}. The tasks where chosen to assess different types of instruction following including specifying: individual objects when there may be duplicates (\textit{e.g.}, an apple on the counter versus one inside a bowl), spatial constraints when placing objects (\textit{e.g.}, placing an onion to the left of a big potato), dealing with occluded objects (\textit{e.g.}, removing a large oil bottle which is blocking the olive oil bottle that needs to be used), and lastly, keeping track of object locations and context as they undergo various manipulations (\textit{e.g.}, taking food off of a dirty plate, washing it, and storing it in the cabinet). Within each condition, the four tasks were assigned in random order. After both condition blocks, participants completed a freeform task to experiment with the features that were excluded from \projname. Details of the individual tasks can be found in the Appendices and Supplementary Material.

\noindent \emph{Measures.} In the study, we collected data on participants' performance when using both methods. Quantitative measures include task completion time and number of errors, which were determined by comparison to an \textit{oracle} representation of the task established \textit{a priori} by two researchers. An error was recorded if: a participant missed a step included in the oracle; there was an extraneous step that was not seen in the oracle; or if a step from the oracle was inefficiently broken into multiple steps by the participant. We also measured subjective perceptions of the prototypes, including participants' confidence in correctly communicating their intent to the robot, workload through the NASA TLX questionnaire~\cite{hart2006nasa}, and system usability (with the System Usability Scale which includes 10 items on a five-point scale~\cite{bangor2008empirical}). Due to data corruption, one task from participant 2 and one task from participant 7 were omitted from the analysis, 

\noindent \emph{Procedure.} Participants first provided consent and completed a pre-study questionnaire assessing their familiarity with robots and instructing them. After watching a video tutorial introducing \projname and the text-based method and brief experimentation with both, participants began one of the two study condition blocks. Between tasks, participants rated how confident they were that the robot could understand their instructions unambiguously on a seven-point Likert scale. At the end of each condition block, two questionnaires (NASA TLX and SUS) were administered to assess workload and usability, respectively. At the end of the study, participants rated their preference for the text-based method compared to \projname on a seven-point Likert scale. Lastly, we conducted a brief interview probing participants about various aspects of both methods.

\noindent \emph{Hypotheses.} We formulated three hypotheses: Participants will complete tasks faster using the \projname compared to the text-based method (\emph{H1}); Participants will make fewer errors using the \projname compared to the text-based method (\emph{H2}); Participants will feel more confident that a robot unambiguously understands their instructions when using \projname compared to the text-based method (\emph{H3}). To test these hypotheses we used a paired t-test for all metrics to account for repeated measures.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/completion_time_with_task_breakdown.png}
%     \caption{Plots showing participants' completion time during the study. The left figure shows the average completion time when one method is shown first (left) versus the other. The figure on the right shows the average completion time of participants broken down by method (image versus text) as well as task.}
%     \label{fig:completion_time}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/results.pdf}    
    \caption{Left: a plot showing the number of errors for both \projname and the Text system. Errors are broken into the three categories extraneous steps, missing steps, and inefficient steps. A bar also displays the total count of all errors. The middle plot shows the task completion time for all 4 tasks, and the completion time across all tasks. Finally at right are the counts of responses for the NASA-TLX questionnaire. All error bars are bootstrapped 95\% confidence intervals.}
    \label{fig:results}
\end{figure*}

\noindent \emph{Findings from Measures of Performance.} \autoref{fig:results} provides a breakdown of participants' completion time by condition and task. Participants were faster (\ttest{37}{-8.96}{0.001}) with \projname ($M=110.8$ seconds, $SD=70.04$ seconds) compared to the text-based method ($M=363.88$ seconds, $SD=186.45$ seconds). 
% Condition ordering affected how much faster participants were able to complete the tasks on average. Condition ordering affected how much faster participants were able to complete the tasks on average. The text-method was much slower ($M=433.7$ seconds, $SD=206.5$ seconds) when seen first versus second ($M=243.5$ seconds, $SD=147.7$ seconds). The same pattern emerged when \projname was seen first, where it was slower ($M=149.0$ seconds, $SD=153.7$ seconds) compared to when it was seen last ($M=89.1$ seconds, $SD=53.5$ seconds).

%The text-method was much slower (M: 433.7s, SD: 206.5s) when seen first versus second (M: 243.5s, SD: 147.7s). The same pattern emerged when \projname was seen first where it was slower (M: 149.0s, SD: 153.7s) compared to when it was seen last (M: 89.1s, SD: 53.5s).

\noindent \emph{Findings from Measures of Error.}. Overall there was no significant difference in errors (\ttestns{37}{-0.76}{0.45}), however \projname ($M=2.26$, $SD=3.07$) had slightly fewer errors than the text-based method ($M=2.55$, $SD=3.02$). The breakdown of errors suggests the text-based method had more (\ttest{37}{-2.43}{0.05}) missing steps ($M=2.0$, $SD=2.11$) than \projname ($M=1.26$, $SD=1.98$). However, there was no difference (\ttestns{37}{1.35}{0.19}) in extraneous steps between \projname () and the text-based method. There was also no significant difference between the text-based method also had fewer inefficient steps ($M=0.38$, $SD=0.92$) than \projname ($M=0.31$, $SD=0.61$).
\noindent \emph{Findings from Measures of Error.}. Overall there was no significant difference in errors (\ttestns{37}{-0.76}{0.45}), however \projname ($M=2.26$, $SD=3.07$) had slightly fewer errors than the text-based method ($M=2.55$, $SD=3.02$). The breakdown of errors suggests the text-based method had more (\ttest{37}{-2.43}{0.05}) missing steps ($M=2.0$, $SD=2.11$) than \projname ($M=1.26$, $SD=1.98$). However, there was no difference (\ttestns{37}{1.35}{0.19}) in extraneous steps between \projname (($M=0.29$, $SD=0.61$)) and the text-based method ($M=0.26$, $SD=0.79$). There was also no significant difference (\ttestns{37}{1.35}{0.19}) between the text-based method ($M=0.26$, $SD=0.79$) and \projname ($M=0.29$, $SD=0.61$) with respect to inefficient steps.

% We are crunching the numbers to determine how ``well'' participants performed at instructing the robot in each task in each condition. Loosely, this means determining where they added extra steps, did not follow the right order of operations (where order matters), and did not follow an instruction correctly. This gives us a metric to quantify how well the user actually did, which is arguably more important than the completion time.

\noindent \emph{Findings from Subjective Measures.} Participants felt more confident (\ttest{37}{5.63}{0.001}) that their instructions would be understood unambiguously by a robot when using the \projname ($M=6.42$, $SD=0.92$) versus the text-based method ($M=4.71$, $SD=1.75$). When comparing system usability, \projname received a higher (\ttest{9}{5.75}{0.001}) average score ($M=87.75$, $SD=14.16$) than the text-based method ($M=61.75$, $SD=23.07$). Lastly, participants reported a lower workload on the NASA TLX when using \projname compared to the text-based method (\autoref{fig:results}). Based on these scores, \projname can be interpreted as having ``excellent'' usability while the text-based mehod would be classified as having ``marginal'' usability. 

%\noindent \emph{Findings from Qualitative Data.} \mk{Things to mention are advantages of image vs text e.g., participant instructions were highly specific.}.

%%%%%% LIMITATIONS OF IMAGE
%%%% PHYSICS IS FAKED
%%%% PEOPLE DO THINGS THEY DON'T KNOW IF THE ROBOT CAN DO RELIABLY

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/tlx.png}
%     \caption{NASA TLX scores from participants for \projname and text-based methods.}
%     \label{fig:nasa-tlx}
% \end{figure}



==> sections/7-real-world-implementation.tex <==
\section{Translating \projname to Robot Actions}
While images may help users specify instructions more easily, they must be possible to execute by the robot. There are potentially various methods to translate images to robot actions, For instance, it could be possible to generate robot policy code~\cite{liang2023code} by processing user-generated images rather than text which could be executed on the robot. We did a preliminary assessment of translation from images to code. To achieve this, we prompt the LLM ten times. As execution performance of the programs are tightly coupled with the robot's skills and environment model (e.g., point cloud quality), we do not assess this. We defined a set of APIs for the robot to use including: \textit{pick}, \textit{place}, \textit{grasp}, and \textit{ungrasp}.

To generate policy code, we prompt an LLM (gpt-4o-2024-05-13) with the predefined APIs, images corresponding to the sequence of steps, the environment, and the environment states (from \projname). We attempted to generate code for two tasks, one simple and two of a medium difficulty both involving sorting fruits. The easy task has two steps requiring the robot to put a red apple in the white bowl (there are two green apples and a red apple on the table). In the medium difficulty task, the green apples should both put in the white bowl while a red apple should be put in the patterned bowl. In the task requiring the robot to put the red apple into the white bowl, the translation was successful 10/10 times. Similarly, the first medium difficulty task involving sorting the apples by bowl type (green apples in the white bowl and red apples in the black bowl), the translation was successful.

Although we did not conduct a thorough assessment of the execution of the code on the robot, we built a pipeline to achieve this using skill primitives (defined earlier). The input parameter to the pick primitive is used to find the relevant environmental object using an open vocabulary object detector (OwLv2~\cite{minderer2024scaling}). This is used to generate an object point cloud by segmenting its 3D bounding box~\cite{kirillov2023segment}, after which sample candidate grasps using Contact-GraspNet~\cite{sundermeyer2021contact}. The place primitive also takes a string description of an object and uses the detector to find and returns a pose for the robot to drop off items.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/robot_execution.pdf}
    \caption{Figure showing the Franka Panda executing code generated by translating images generated with the \projname interface.}
    \label{fig:robot_execution}
\end{figure}


==> sections/8-discussion.tex <==
\section{Discussion}
\noindent \emph{Contextualizing the performance of \projname.} The results of our user evaluation suggest that \projname led to faster completion of the instruction giving tasks with fewer errors. Specifically, participants had more missing steps when they used the text-based method. One rationale could be that images support keeping track of the environment state over longer-horizon tasks so they were less likely to miss a step, However, participants included more extraneous steps (i.e., steps that do not contribute to the goal) possibly due to the low cost of adding new instructions afforded by direct manipulation. 

Several factors that could lead to participants spending significantly more time and effort giving instructions in language.
We notice that the additional cost of using the text-only modality were more pronounced in resolving ambiguities, for example, when referencing specific objects or achieving precise object placement.
P9 commented ``\textit{The text interface was incredibly cumbersome...Because the room for ambiguity in the instructions made it so that each step required a lot of mental processing to try to remove any ambiguities in my instruction.}''
Participants often needed to use complex referring expressions when trying to disambiguate between multiple similar objects, whereas with \projname they could select the target object directly. 
In a similar vein, participants often had to construct complex sentences to describe the exact locations for objects to be placed.
Apart from these two types of instructions, participants also reported challenges in error correction with text, as it requires to ``\textit{create a series (of new instructions)}'' (P4).

Participants noted the extraneous cognitive effort for making sense of multi-step plans as they get longer in the text-based condition. 
They talked about the difficulty in mentally tracking object location and state changes, and how it negatively impacted their confidence in their instructions.
Further, they liked the immediate visual feedback that \projname affords to help them evaluate action feasibility and plan further, contrasting it with the text-based condition where ``\textit{I have to imagine what the result of this (text-based) is going to be... it's like playing a game of blindfolded chess.}'' (P6). 

%%%%% MENTION HOW IMAGES STAY THE SAME LENGTH REGARDLESS OF INSTRUCTION SPECIFICTIY WHILE OTHER METHODS LIKE LANG DO NOT

%%%%%% IMAGES ARE EASIER TO KEEP TRACK OF WHAT'S GOING ON (WHOLE ENV STATE IS DESCRIBED IN IMAGE). YOU CAN DO THAT WITH TEXT BUT IT WOULD TAKE FOREVER.

%%%%%% REFERENCING SPECIFIC OBJECTS IS VERY SIMPLE (AMBIGUITY)

%%%%%%%%%%%%%% PLACING THINGS PRECISELY IS STRAIGHFFORWARD (TEXT YOU HAVE TO MAKE A TRADEOFF LIKE WRITING MORE TO BE MORE PRECISE).

\noindent \emph{Limitations.} Though we are encouraged by the findings that participants made fewer errors, there are some caveats. First, our comparison required participants to provide step-by-step instructions for a robot when using the text-based method. While this is how robots act on instructions, humans may think at higher abstraction levels. Here, there is the potential for LLMs to take a higher-level instruction and break it down into a sequence of lower-level instructions for the robot, though these are prone to errors~\cite{zha2023distilling}. Hence, we note that the performance of \projname represents the best-case scenario for the image manipulation paradigm and the worst-case scenario for the text-based method (\autoref{fig:results}). Technical limitations also bound \projname's performance, including that of the underlying models for detecting objects reliably, masking them into meaningful objects, and the ability for vision language models to perceive environment changes. In particular, 2D editing could sometimes be affected by the problem of perspective. When objects are manipulated, they tend to change size and appear out of place which may impact detection or recognition performance.

%%%% MENTION THAT IMAGES DON'T DEAL WITH PERSPECTIVES AND ARE MORE CONCRETE AS LIMITATIONS

%%%% OTHER MODELS CAN CAUSE ISSUES TOO LIKE DETECTING AN OBJECT INCORRECTLY (E.G., SODA BOTTLE AS SYRUP BOTTLE, ETC.)

\noindent \emph{Future Work.}
Although there is some early evidence that user-manipulated images could be translated into robot code, it is preliminary. It would be important to thoroughly assess where image manipulation can succeed and where it has shortcomings. For instance, we noticed (anecdotally) that vision language models find it challenging to describe small changes (e.g., when a bowl shifts a bit to one direction or another). Further, we would like to assess how robot foundation models---particularly those that condition on goal images would perform if provided user-manipulated images since these would likely be out of their training distribution (as image manipulation inherently leads to awkward object scaling and perspective). Lastly, it would be interesting to explore whether interaction traces when using systems like \projname can be leveraged to learn user patterns and preferences for tasks. For instance, observing the user put heavier dishes on lower shelves could prompt similar suggestions or better initial proposed steps from the system.

%%%%% Showing translation more thoroughly; across more tasks and between translation types (e.g., image to image or image to text)

%%%% Learning from user traces as context 

% \noindent \emph{Real-world usage of \projname.} We believe that the workflow for a user interacting with \projname will incorporate \textit{multimodal instructions}. Suppose the user has just hosted a party and wants their robot to help clean the dishes (akin to the \textit{Washing Dishes} task in \autoref{fig:tasks}). Upon pulling up the \projname interface, instead of multiple drag-and-drop manipulations, the user would begin by typing their higher level goal of washing the dishes. This prompts \projname to break down the task step-by-step and generate images of the proposed instructions. For instance, the steps may involve the robot rinsing and stacking each cup on top of the dry cups. Upon noticing this, the user can manipulate the cups away so that they are not making contact with the dry cups.\mk{}.

% Case study
% Suppose a user is creating a program for a
% social robot providing general assistance in a public area. Here,
% the robot may have states such as idle, greeting, or thinking. The
% user can begin by creating state nodes within the state editor. One
% such state could be labeled “Idle” to represent the idle status of the
% robot within the overall program. From here the user can begin
% adding Behavior Properties to the state. First, the user may apply
% the Position Liveliness property to the torso of Pepper as a visual
% indication that it is powered-on and functioning. Next, the user may

% add the Joint Liveliness property, and confgure it to “Head Yaw” to
% make the robot’s head sway from left to right and signify that it
% is looking around for people to assist. Finally, the user can select
% the Smoothness Macro property to ensure that the robot’s motion
% remains smooth and natural, and the Collision Avoidance property
% to prevent collisions. The user may also create a "Greeting" state,
% which directs the robot’s gaze toward a nearby person. Once these
% states are generated, the user can create a connection between
% them and add a label to identify a triggering condition. The user
% may want Pepper to transition from the "Idle" state to a "Greeting"
% state when a person approaches. During this transition, Pepper can
% reduce head sway from the "Idle" state, direct gaze toward the user
% in the "Greeting" state, and maintain the liveliness motion included
% in both states. This process can be repeated with any number of
% states and complex transition patterns.


==> sections/9-conclusion.tex <==
%%%% LIMITATIONS
%%%%%%%%%% PERSPECTIVE
%%%%%%%%%% LACK OF CONT. ACTION SPACES (ONLY DISCRETE FOR NOW)
\section{Conclusion}
In this work, we proposed the direct manipulation of images as a new paradigm for robot instruction, and showed its feasibility and capabilities through our prototype system, \projname. Through user studies comparing \projname with a text-based baseline across four complex kitchen manipulation tasks, we have shown that image manipulation enables the quick specification of robot instructions with less effort and workload. Through this work, we also took a step towards future interfaces that blend image and language seamlessly as each modality has their benefits (such as being able to be abstract or repeat an instruction many times with language). This multimodal form of instruction could benefit users with differing capabilities and needs.We hope that this inspires significant future efforts towards methods that support humans in instructing robots.

% The interface design of \projname allows for a blended use of both image and language, and our study results also suggest the complementary strengths of image to language commands. 
% Beyond proposing image manipulation as a useful modality for instructing robots, we would like to highlight its potential role in future multimodal HRI, where both images and languages can be flexibily transformed into one another as commands and robot program representations, depending on the demands of the users and tasks.    

% \projname supports direct manipulation of objects and fixtures in images of a robot's operating environment as an efficient and low-ambiguity way for users to express their intents.
% By representing instructions as a series of images, \projname allows users to visually track robots' planned action, reducing the cognitive effort for commanding robots in long-horizon tasks.


% Summary. In this work, we proposed an approach, GenEM, to
% generate and modify expressive robot motions using large language
% models by translating user language instructions to robot code.
% Through user studies and experiments, we have shown that our
% framework can quickly produce expressive behaviors by way of
% in-context learning and few-shot prompting. This reduces the need
% for curated datasets to generate specific robot behaviors or carefully
% crafted rules as in prior work. In the user studies, we demonstrated
% that participants found the behaviors generated using GenEM with
% user feedback competent and easy to understand, and in some cases
% perceived significantly more positively than the behaviors created
% by an expert animator. We have also shown that our approach is
% adaptable to varying types of user feedback, and that more complex
% behaviors can be composed by combining simpler, learned behaviors.
% Together, they form the basis for the rapid creation of expressive
% robot behaviors conditioned on human preferences.

==> sections/old/2-related-work.tex <==
\section{Related Work}
Prior research has explored a range of approaches for robot control.
These include systems focusing on creating reusable, repeatable routines (i.e., using end-user robot programming (EURP) and techniques for interpreting humans' low-level (e.g., teleoperation) and high-level (e.g. language) commands for robot actions.
This research has been built on the work in these spaces.
%Our system falls somewhere in between, blending elements of both approaches.

\noindent \emph{End-user robot programming.} Prior EURP work can be largely categorized into natural language-based and visual-based methods. Many systems employ speech for programming~\cite{cakmak2014teaching, gorostiza2011end}, though challenges remain in recognition and creating complex programs through continuous dialogue. Other approaches use text-based programming with visual scaffolds like blocks~\cite{huang2017code3, huang2016design, weintrop2018evaluating} or nodes~\cite{alexandrova2015roboflow,porfirio2018authoring}. Recently, large language models (LLMs) have been employed for text-based interactions, often via chat interfaces~\cite{karli2024alchemist, ge2024cocobo}. However, language input demands precision, especially for spatial tasks in robotics~\cite{masson2024directgpt, sundaresan2024rt}. Other systems span a range of visual modalities, such as augmented reality~\cite{ikeda2024programar, suzuki2022augmented, quintero2018robot, gong2019projection, cao2019ghostar}, spatial interfaces~\cite{huang2020vipo, cao2019v, mahadevan2022mimic}, sketch-based systems~\cite{sakamoto2009sketch, porfirio2023sketching}, physical demonstrations~\cite{akgun2012trajectories}, and tangible interaction~\cite{sefidgar2017situated, gao2019pati}. Despite the richness of prior EURP systems, they often require adherence to specific system rules. For instance, AR-based trigger-action programming~\cite{ikeda2024programar} necessitates precise trigger and action specifications within the user's AR environment. Moreover, many prior systems use intermediate representations (e.g., flow diagrams or blocks) to convey user intent. In contrast, \projname enables users to directly manipulate images to represent a desired world state without an intermediate representation.

% Mention ~\cite{li2022scene} at some point.

% FrameKit: A Tool for Authoring Adaptive User Interfaces Using
% Keyframes

% Montage: A Video Prototyping System to Reduce
% Re-Shooting and Increase Re-Usability

% Gaze+Hold: Eyes-only Direct Manipulation with Continuous
% Gaze Modulated by Closure of One Eye

% Authoring Sensor-based Interactions by Demonstration
% with Direct Manipulation and Pattern Recognition

% Multimodal Direct Manipulation in Video Conferencing:
% Challenges and Opportunities

% Representation
% Blocks: Code3 ~\autoref{huang2017code3, huang2016design, weintrop2018evaluating}
% Natural language: Alchemist ~\autoref{karli2024alchemist, ge2024cocobo}
% Spatio-visual: ~\autoref{huang2020vipo, senft2021situated}
% Demonstration + visual: ~\autoref{mahadevan2022mimic, porfirio2019bodystorming}

%% Augmented reality: ~\autoref{ikeda2024programar, suzuki2022augmented, quintero2018robot, gong2019projection, cao2019ghostar}
%% Tangible: ~\autoref{sefidgar2017situated, gao2019pati}
%% Sketch: ~\autoref{porfirio2023sketching, sakamoto2009sketch}

% Things to mention
% - the type of representations thaat people use like block/tangible/etc.
% - types of logic that programming has supported: loops/conditionals/
% - granularity of program: low vs high level

%https://dl.acm.org/doi/pdf/10.1145/2909824.3020249

% \cite{huang2022inner} also explores the idea of using feedback but the feedback can come from several sources like automated success detectors, scene descriptors like object detection modules, and human feedback. Precursor to works like distillation but still valid and relevant.

%\cite{yao2022react} A generalist paper that is talking about how LLMs on the whole can use language feedback to modify task-level step-by-step plans

% \cite{yu2023language} Also talks about using language but to generate rewards for robot skills. Similar to mine but uses a module to generate rewards and a motion controller instead of APIs.

% \cite{kwon2023toward} Use VLM and LLM loops to reason about things in a visual manner. In this manner, it is sort of suggesting that we don't necessarily need humans as much, but still a point towards visual information matters. Probably can borrow their motivation portions. In fact, they answer the question about commonsense but state clearly that somethings (and they have proof with user studies) are subjective like dirtiness. They even show that this improves overall grounded reasoning.

% \cite{hunt2024survey} Read and include if necessary.

% \subsection{End-User Robot Programming}
% %Can model after 2.2 of https://arxiv.org/pdf/2406.00841.
% End-user robot programming (EURP) aims to allow non-coders to program robot behaviors~\cite{lieberman2006end,ajaykumar2021survey}.
% Early EURP tools tapped into showing users graphical representations of robot programs, such as flow diagrams~\cite{alexandrova2015roboflow,porfirio2018authoring}.
% As these methods still require users to have some levels of understanding about a robot's available low-level actions, other work looked into programming robots by directly demonstrating desired behaviors through kinethestic teaching~\cite{akgun2012trajectories} or teleoperation~\cite{kitagawa2023online}.
% Another line of work explored using visual mark-ups on environments to set robot trajectories and points of interests~\cite{cao2019v,liu2011roboshop}.  
% However, these methods could not directly capture people's high-level goals, requiring them to sometimes arduously specifying individual actions.
% One exception is RT-Sketch~\cite{sundaresan2024rt}, which could interpret high-level state change goals from users' sketches of desired world states.
% However, as these sketches only captured object contours, they are limited in expressing object articulation and distinguishing similar objects.

% Recent advances in AI has enabled users to program high-level robot behaviors through natural language~\cite{tellex2011understanding,liang2023code,winge2024talk}.
% While expressive, natural language commands come with ambiguity that makes programming often more effortful than expected~\cite{stegner2024understanding}.
% Some recent work combined visual editing with natural language input to resolve ambiguity and simplify verbal expressions~\cite{porfirio2023sketching}.
% This research builds on existing work that leverages the complementary strengths of language and visual editing, and expands the expressiveness of visual editing by introducing object manipulation and state change generation.

% \subsection{Human-in-the-Loop Robot Planning}
% With the advent of robot foundation models, end-users may not need to program their robots completely from scratch as many prior systems assume. Instead, the end user's role may be to steer the model to plan towards their desired goals. Prior work has explored human-in-the-loop planning approaches to correct robots acting autonomously. In these settings, language has been seen as a natural fit to express user corrections or clarifications. For instance, it has been used to provide iterative corrections~\cite{zha2023distilling} that the robot can distill knowledge from in a future task (e.g., how to set a table) or to accelerate learning from specific users~\cite{liang2024learning}. It has been used to generate reward functions~\cite{yu2023language} or code~\cite{mahadevan2022mimic} to generate social robot behaviors. \projname enables user manipulations on images to refine and correct robot plans.

\noindent \emph{Live robot control.} Modern robotic systems often include interfaces for the real-time teleoperation of the robots' joint and end-effector positions.
These interfaces are often based on graphical user interfaces (GUIs) or joysticks, offering immediate feedback for the controllers to adjust their input~\cite{darvish2023teleoperation,rea2022still}.
While effective, GUI- and joystick-based control mechanisms are cognitively and physically taxing for human operators, as they demands mental rotation and managing multiple separate degrees of freedom (DoFs) simultaneously.
To alleviate this burden, one thread of recent teleoperation research aims to directly map human motion to robot motion, often from the motion of human hands to robot end-effectors~\cite{rakita2017motion,rakita2019shared,fu2024mobile}.
Other work opts for a shared-control approach, where some trajectory prior informs a robot to generate high DoF trajectories from low DoF input.
Such prior is often derived from inferred operator goals~\cite{huang2016anticipatory,jain2019probabilistic,losey2022learning}.
Despite the assistance available, live control methods still require operators' continuous mental and physical engagement to manage robots' low-level motion.
Therefore, \projname, along with other recent research, seeks to enable robots to interpret and execute human operators' high level intents.


\noindent \emph{Helping robots follow human instructions.} With the advent of foundation models (FM), end-users may not need to program their robots from scratch (as with EURP). Recent work has successfully deployed pre-trained LLMs for robotics tasks such as translating language instructions to policy code~\cite{liang2023code, singh2023progprompt, liu2024ok, mahadevan2024generative}. Previous work has demonstrated that language can be used to iteratively guide and correct robots, enabling them to learn from these interactions and apply that knowledge in future tasks~\cite{zha2023distilling, liang2024learning}. In contrast, other work has attempted to translate human instructions into robot actions directly by training robotic foundation models (RFM~\cite{kawaharazuka2024real}). Some of these techniques can generate actions when provided natural language inputs~\cite{driess2023palm, kim2024openvla}, such as, ``Bring me the chips from the drawer''. Alternatively, images can be used to represent goals, either as sub-steps of a task~\cite{black2023zero, nair2020contextual} or the final desired state~\cite{team2024octo, kapelyukh2023dall}. There are also attempts at using other modalities, including representing goals as sketches~\cite{sundaresan2024rt}, or desired trajectories overlaid on images~\cite{gu2023rt}. Our framework realized through \projname, is agnostic to the method used to provide instructions to the robot. This flexibility is achieved by separating the user's input representation when providing instructions from the representation used to execute the instructions. For example, images can be captioned and sent as language instructions to a language-conditioned RFM. Alternatively, pre-trained models can translate images into executable code using existing skill primitives (e.g., picking up a coffee mug). The images can also be directly provided to an image-conditioned RFM.

%Prior work has shown that image-conditioned policies currently outperform language-conditioned policies~\cite{team2024octo} possibly as images inherently contain more concrete information about how to perform a task in a given environment. Our work, \projname, is partially motivated by the need to create images to serve as an input for goal-conditioned robot policies.

%To our knowledge, prior work (with the exception of RT-Sketch~\cite{sundaresan2024rt}) has assumed that goals can be autonomously generated (e.g., as in \cite{black2023zero}) to handle users' language instructions. This can be problematic both due to artifacts (an inherent limitation of diffusion models) and difficulties in precisely translating language instructions into images representing the user's desired goals. In contrast, we introduce \projname as a method to enable users to directly create images that represent sub-steps that a robot should execute using image-conditioned robot policies.

%\cite{winge2024talk} Kind of relevant with the idea of end user adaptation of an existing robotic system but really not that interesting.

%\cite{stegner2024understanding} Generalist paper about on-the-fly EURP. Might be able to refer to some of the challenges when talking about our solution (though we aren't fully building an EURP but it is the building blocks towards it to an extent).
%e.g. Theme 1: End users viewed program steps to better understand the system: Relevant because we allow this
%e.g. heme 4: End users had mixed experiences on interaction with the program synthesizer: Want to ensure our system provides users a sense of being in control
%\mk{Talk about EURP work that uses image editing/sketch/environment editing.}
%\cite{liu2011roboshop,skubic2007using} sketch-based interface for mobile robot control (little manipulation).
%\cite{sundaresan2024rt} allows users to draw object contours to specify desired environmental changes. 


%\cite{} Survey on EURP so regardless of anything we'd need to cite it.

% \subsection{Interfaces for Authoring and Browsing Spatial Content}
% Our prototype of \projname is directly inspired by significant HCI research into developing direct manipulation interfaces as well as interaction techniques for editing using keyframes.

% \emph{Direct manipulation.} Prior work in HCI has explored the use of direct manipulation, an interaction style where objects of the interface can be interacted with via physical, reversible, and incremental actions and that provide immediate feedback~\cite{shneiderman1982future, shneiderman1983direct}. For instance, videos can be scrubbed by directly manipulating the content rather than the timeline~\cite{dragicevic2008video, karrer2008dragon}. Direct manipulation has also been used to support the navigation of 3D spatial recordings~\cite{lilija2020put, xia2018spacetime}. It has been used to support drawing tools to visualize data~\cite{xia2018dataink, kim2019datatoon}, make procedural art~\cite{jacobs2017supporting}, programming SVGs~\cite{hempel2016semi}, and creating illustrations~\cite{xia2016object}. Direct manipulation has seen some application in robotics, including for programming robot swarms~\cite{suzuki2018reactile, le2016zooids, suzuki2019shapebots}, and to teleoperate a robot by manipulating a virtual scene~\cite{li2022scene}. Our prototype, \projname, enables the direct manipulation of images to facilitate robot program creation.

% \emph{Keyframe editing.} Prior work has investigated the design of interfaces that enable users to add keyframes to express moments of change in authoring and consumption tools. The idea has been extensively used for video browsing via extracted keyframes~\cite{huber2010toward, tse1998dynamic}. It has also been employed for creating animations~\cite{koyama2018optimo, zhou2024timetunnel, tseng2024keyframer} as well as the design of websites manually~\cite{krosnick2018expresso} or through computational assistance~\cite{wu2024framekit}. In \projname, all intermediate steps are represented as keyframes that can be quickly navigated, modified, and cloned.

% \begin{figure}[t]
%     \centering
%     \missingfigure[figwidth=\linewidth]{Insert background figure}
%     % \includegraphics[width=\linewidth]{figures/background-figure/background-figure.v01.png}
%     \caption{
%         \mk{Background figure.}
%         \textnormal{Some caption}
%     }
%     \label{fig:background}
%     % \vspace{-8mm}
% \end{figure}


%\bla{there is a commented out attempt at framing this as background and related work below here.}

%\bla{The goal of the rewrite is to argue that all forms of robot instruction (end user programming, instruction following, live control, etc.) rely on some form of instruction representation. We do not want our work to be seen as end user programming, and it's definitely not live control. But we don't want to introduce our own paradigm. That's a big leap. Instead, we introduce the abstract notion of \textit{Instruction Representation}, which covers many of these areas, and argue that there are three important aspects namely: creation, interpretation, and execution. And then we can argue that representing instructions as images has key benefits, and those benefits might apply to other paradigms as well.}
% The HRI literature includes several paradigms in which a human might instruct a robot. For example, humans might use *teleoperation* where they are interacting in real time and directly controlling the robots movement, or *live control* which is also done synchronously in real-time, however the method used to control the robot is typically abstracted, perhaps using instruction following and voice to control the robot and give language based commands. The feedback loop in these cases is so tightly integrated that the instructions are usually not represented to the user in any other way than by using an image of the environment. These approaches are rooted in the real-time nature. 

% However, our application domain attempts to address problems in the household where a user might want to offload tasks. If these were done in real time with a human in the loop then it is difficult to imagine the user would be saving time. Some paradigms have attempted instruct robots in a non-real time manner. For example, end-user robotics programming tries to create reusable programs that the robot can execute. 

% Our paper does not fit directly into any of these paradigms, and instead represents a combination of many of them. We take from the end user programming literature the idea of constructing many consecutive steps, but from instruction following and live control we take the representation of instructions. It is unclear where this new paradigm sits, but it is somewhere at the intersection of end user robotics programming and instruction following. 

% We present a small model and mini taxonomy in which these paradigms fit into, and argue that beyond these paradigms there is a generalisable concept regarding robot instruction. Whether the user is trying to program the robot, live control it, or use instruction following, the instruction the user is conveying MUST be created and represented in some manner. Teleoperation uses a live video, end user programming ranges from using blockbased programming, instruction following creates the representation with voice and interprets it with sound or written text. In this paper we use a static 2D image of the environment both to manipulate and create instructions for the robot.

% In the remaining background and related work we discuss the projects which are most similar to our work, and a brief survey of different methods of the modalities used to create, represent, and execute instructions.

==> sections/old/3-theory.tex <==
\section{Theory and Design Space}
\subsection{Why Use Images?}
Thus far, we have motivated the use of images to serve as goals for policies enabled by robot foundation models. Here, we motivate why images are useful as a representation for both visualizing their desired goals as well as to manipulate them.

\bla{I think we should use the terminology ``interpretation'' and ``creation'' it's inherently human, robots don't interpret or create things, and the terms input and output are fraught with misunderstandings.}

\noindent \emph{As an output representation.} For the user, visually being able to inspect the robot's environment (either in physical form or as images) can make it easier to ground themselves when providing instructions. Beyond this, being able to quickly inspect sub-steps of a program could help them spot errors before they occur, when compared to a step-by-step language procedure which may be more difficult to scan especially if the steps contain long instructions.

\noindent \emph{As an input representation.} When instructing a robot using language, user intent may be hard to convey due to ambiguities associated with language~\cite{masson2024directgpt, sundaresan2024rt}. For instance, when setting a table, simply saying ``put the plate and utensils on the table'' is not sufficient because it does not detail where the items should be placed (in absolute terms) or with respect to each other (in relative terms). In this case, the user needs to precisely phrase their instruction to describe the task but in a way that can be understood by the system (e.g., ``put the fork to the left of the plate but center it vertically''). 

In contrast, images more concretely describe a desired outcome with less room for interpretation (e.g., putting the fork to the left of the plate and aligning it vertically). However, a major challenge lies in how to generate goal images for the robot to execute~\cite{sundaresan2024rt}. While prior work has shown that this can be achieved through autonomous methods (e.g., \cite{black2023zero}), such methods currently suffer from generating images with artifacts. Further, text-to-image models still struggle with the same problems of ambiguity along with needing to specify what parts of an image need to change and what parts need to stay the same. 

We think that direct manipulation could make it possible to quickly create images that more accurately capture a user's desired goals. For instance, through a simple drag-and-drop, the user can position a fork to the left of a plate to convey both absolute and relative positioning of the objects. Further, we think that the user's interactions with task-relevant objects of the environment through an image could make it possible to make inferences about their intent. For instance, dragging a dirty bowl from the dining table to the sink could signal that other utensils nearby might also need cleaning.

\subsection{Program Representation as Images}

\subsection{Model of Program Creation}

\bla{If we have room I'd like a figure of this process.}

There are many steps involved in the process of instructing a robot. The user must be able to create the instructions, interpret those instructions, and evaluate the effect of the instructions. The robot must execute the instructions. In this paper we focus on the process of creating and interpreting instructions for robots. 

% what are the pros and cons of different methods in detail? What does the user want? Focus and scope into what the user wants for everyday household tasks. 
